A Robust Feature-aware Sparse Mesh Representation

The sparse representation of signals defined on Euclidean domains has been successfully applied in signal processing. Bringing the power of sparse representations to non-regular domains is still a challenge, but promising approaches have started emerging recently. In this paper, we investigate the problem of sparsely representing discrete surfaces and propose a new representation that is capable of providing tools for solving different geometry processing problems. The sparse discrete surface representation is obtained by combining innovative approaches into an integrated method. First, to deal with irregular mesh domains, we devised a new way to subdivide discrete meshes into a set of patches using a feature-aware seed sampling. Second, we achieve good surface approximation with over-fitting control by combining the power of a continuous global dictionary representation with a modified Orthogonal Marching Pursuit. The discrete surface approximation results produced were able to preserve the shape features while being robust to over-fitting. Our results show that the method is quite promising for applications like surface re-sampling and mesh compression.

==> algorithms/create_patch.tex <==
\begin{algorithmic}[1]
    \REQUIRE Let $s$ be the center point.
    \REQUIRE Let $\set{T}$ be a set of neighboring triangles of $s$ with increasing distance.
    \ENSURE Final set $\Patch$ of patch points.
	\STATE $\Patch = s$
	\FOR{ $t = \set{T}_1, \set{T}_2, \set{T}_3, \ldots$ }
	\IF{ $t$ satisfies conditions $\set{C}$ }
	    \STATE $\Patch = \Patch \cup \{t\}$
	\ENDIF
	\ENDFOR
	\RETURN $\Patch$ 
\end{algorithmic}


==> algorithms/sampling.tex <==
\begin{algorithmic}[1]
    \REQUIRE Set $\set{I}$ of interest points sorted by increasing values of featureness (Harris3D saliency).
    \ENSURE Final set $\Seeds$ of seed points.
	%\STATE $max\_radio = Fast\_Marching(I)$
	\STATE $\Seeds = \emptyset$ 
	\FOR{ $p = \set{I}_1, \set{I}_2, \set{I}_3, \ldots$ }
	\IF{ $\displaystyle\min_{q \in \Seeds} \norm{p - q} \ > \ \sigma \cdot r_q$ \textbf{or} $\Seeds == \emptyset$}
	\STATE $\Patch = patch\_construction(p)$ 
	    \IF{ $\Patch \neq \emptyset$ }
	    \STATE $ \Seeds = \Seeds \cup \{p\} $
	    \STATE $ \displaystyle  r_p = \max_{q \in \Patch} \ \norm{p - q}$
	    \ENDIF
	\ENDIF
	\ENDFOR
	\RETURN $\Seeds$ 
\end{algorithmic}


==> tables/comparison.tex <==
\begin{tabular}{|l|c|c|c|c|c|}	\hline
\textbf{Mesh}	&	\textbf{n}	&	\textbf{M}	&	\textbf{$\rho$}	&	\textbf{RMSE}	&	\textbf{C.R.}	\\\hline
fandisk	&	6475	&	540	&	0.001	&	0.0001266	&	0.6147	\\
torus	&	14400	&	596	&	0.005	&	0.0003436	&	0.3449	\\
kitten	&	43544	&	1680	&	0.0002	&	0.0004092	&	0.3215	\\
bunny	&	72027	&	4301	&	0.0001	&	0.0003269	&	0.4976	\\
armadillo	&	172974	&	10323	&	0.0001	&	0.0001895	&	0.4973	\\
kitten	&	172974	&	10323	&	0.0001	&	0.0005664	&	0.4973	\\
SH109	&	49127	&	5749	&	0.0005	&	0.0004192	&	0.8625	\\
SH165	&	49929	&	5578	&	0.0005	&	0.0008189	&	0.8303	\\
SH170	&	49956	&	4742	&	0.0005	&	0.0011380	&	0.7265	\\
SH202	&	49982	&	4239	&	0.0002	&	0.0003717	&	0.6897	\\
SH72	&	49982	&	4266	&	0.0002	&	0.0003266	&	0.6994	\\\hline
\end{tabular}
